Spider: Any-to-Many Multimodal LLM

Multimodal LLMs (MLLMs) have emerged as an extension of Large Language Models (LLMs), enabling the integration of various modalities. However, Any-to-Any MLLMs are limited to generating pairwise modalities 'Text + X' within a single response, such as Text + {Image or Audio or Video}. To address this limitation, we introduce Spider, a novel efficient Any-to-Many Modalities Generation (AMMG) framework, which can generate an arbitrary combination of modalities 'Text + Xs', such as Text + {Image and Audio and Video}. To achieve efficient AMMG, our Spider integrates three core components: a Base Model for basic X-to-X (i.e., Any-to-Any) modality processing, an Any-to-Many Instruction Template designed for producing Xs signal prompts, and a novel Efficient Decoders-Controller for controlling multimodal Decoders to generate Xs (many-modal) contents. To train Spider, we constructed a novel Text-formatted Many-Modal (TMM) dataset, which facilitates learning the X-to-Xs (i.e., Any-to-Many) capability necessary for AMMG. Ultimately, the well-trained Spider generates a pseudo X-to-Xs dataset, the first-ever X-to-Xs many-modal dataset, enhancing the potential for AMMG tasks in future research. Overall, this work not only pushes the boundary of multimodal interaction but also provides rich data support for advancing the field. Code: https://github.com/Layjins/Spider

==> sec/2_relatedwork.tex <==
\section{Related Work}
To build foundational Multimodal LLMs (MLLMs), researchers align pre-trained encoders from various modalities with the textual space of LLMs, enabling them to process multimodal inputs \cite{huang2023language, zhu2023minigpt, su2022language, koh2023generating, alayrac2022flamingo, li2023blip, liu2023visual}. 
%For example, Flamingo \cite{alayrac2022flamingo} connects a fixed image encoder to LLMs using cross-attention, while LLaVA \cite{liu2023visual} links image and word spaces via projection. BLIP-2 \cite{li2023blip} uses a Q-Former to translate image queries into LLMs. 
%Similar approaches are applied to videos (e.g., Video-Chat \cite{li2023videochat}, Video-LLaMA \cite{zhang2023video}) and audios (e.g., SpeechGPT \cite{zhang2023speechgpt}). 
PandaGPT \cite{su2023pandagpt} extends input with six modalities using ImageBind \cite{girdhar2023imagebind}.
Approaches like Visual-ChatGPT \cite{wu2023visual}, HuggingGPT \cite{shen2023hugginggpt}, and AudioGPT \cite{huang2023audiogpt} use LLMs as decision-makers, incorporating external multimodal encoders and decoders for multimodal input-output. Despite this, discrete text-message-based pipelines can introduce noise and hinder semantic understanding. NExT-GPT \cite{wu2023next} overcomes this by learning an end-to-end multimodal input-output LLM, capable of handling any combination of text, image, video, and audio.
However, these X-to-X MLLMs are limited to generating pairwise modalities 'Text + X' within a single interaction.
In contrast, our proposed X-to-Xs Spider model aims for Any-to-Many Modalities Generation in a single response, supporting arbitrary combinations of a wider range of modalities as shown in Fig.~\ref{fig:supported_x}, including text, image, audio, video, box, and mask.
